Top-Quark Physics at the CLIC Electron-Positron Linear Collider

The Compact Linear Collider (CLIC) is a proposed future high-luminosity linear electron-positron collider operating at three energy stages, with nominal centre-of-mass energies: 380 GeV, 1.5 TeV, and 3 TeV. Its aim is to explore the energy frontier, providing sensitivity to physics beyond the Standard Model (BSM) and precision measurements of Standard Model processes with an emphasis on Higgs boson and top-quark physics. The opportunities for top-quark physics at CLIC are discussed in this paper. The initial stage of operation focuses on top-quark pair production measurements, as well as the search for rare flavour-changing neutral current (FCNC) top-quark decays. It also includes a top-quark pair production threshold scan around 350 GeV which provides a precise measurement of the top-quark mass in a well-defined theoretical framework. At the higher-energy stages, studies are made of top-quark pairs produced in association with other particles. A study of ttH production including the extraction of the top Yukawa coupling is presented as well as a study of vector boson fusion (VBF) production, which gives direct access to high-energy electroweak interactions. Operation above 1 TeV leads to more highly collimated jet environments where dedicated methods are used to analyse the jet constituents. These techniques enable studies of the top-quark pair production, and hence the sensitivity to BSM physics, to be extended to higher energies. This paper also includes phenomenological interpretations that may be performed using the results from the extensive top-quark physics programme at CLIC.

==> utilities/packages.tex <==
\usepackage{lipsum}

\RequirePackage[T1]{fontenc}

%line number
\usepackage{lineno}

%\smartqed  % flush right qed marks, e.g. at end of proof

%\usepackage{draftwatermark}
%\SetWatermarkFontSize{1.8cm}
%\input{globalrevision.tex}

\RequirePackage{color}
\RequirePackage{graphicx}
\RequirePackage{mathptmx}      % use Times fonts if available on your TeX system
\RequirePackage{flushend}
\RequirePackage{feynmp}
\RequirePackage{amsmath}
\RequirePackage{heppennames2}
\RequirePackage[numbers,sort&compress]{natbib}

\usepackage{bm}
\usepackage{amsmath,slashed}
\usepackage{amssymb}
\usepackage{tocloft}
\usepackage{texnames}
\usepackage[T1]{fontenc}
\pagestyle{plain}
\usepackage{color}

\usepackage{footmisc}

%\usepackage[square,numbers,sort]{natbib}
\usepackage{url}

%\usepackage{draftwatermark}
%\SetWatermarkFontSize{1.8cm}

\usepackage{units}
\usepackage{siunitx}
\usepackage{booktabs}
%\usepackage{subfig}
\usepackage{subcaption}
\usepackage{graphicx}
%\usepackage{feynmp}
\usepackage{feynmp-auto}
\DeclareGraphicsRule{*}{mps}{*}{}

\usepackage{adjustbox}

%For tables
\usepackage{multirow}

%%For title layout
\usepackage{textpos} % for placement of logo 
\usepackage{relsize} 

%%Font treatment
\usepackage{mathptmx}
\usepackage[scaled=.90]{helvet}
\usepackage{courier}
\usepackage[T1]{fontenc} %font enconding
\usepackage[latin9]{inputenc} %input encoding


%%Layout spacing

% align left the itemize and enumerate lists, and reduce space
\usepackage{enumitem}
\setlist{noitemsep}
\setlist[itemize]{leftmargin=*, topsep=-2pt, partopsep=0pt, itemsep=2pt}
\setlist[enumerate]{leftmargin=*, topsep=0pt, partopsep=0pt, itemsep=0pt}

% no paragraph indentation
\setlength{\parindent}{0pt}
\setlength{\parskip}{1.3ex} % less space between paragraphs


% hyper ref and cleverer needs to be last
%\RequirePackage[colorlinks,breaklinks,citecolor=blue,urlcolor=blue,linkcolor=blue]{hyperref}
\renewcommand*{\sectionautorefname}{Section}
% \hypersetup{draft}
\urlstyle{same}
% fix bug in svjour3 (only happens with cleverer)
\makeatletter
%\def\cl@chapter{\cl@chapter \@elt {theorem}}%bug in class
\def\cl@chapter{\@elt {theorem}}
\makeatother

\let\subsectionautorefname\sectionautorefname
\let\subsubsectionautorefname\sectionautorefname

\RequirePackage[capitalize]{cleveref}

%TODO list
\usepackage[colorinlistoftodos]{todonotes}

%============================================%
% Additional units and configuration
%============================================%
\sisetup{
  separate-uncertainty=true, % write 5.3+-0.2 instead of 5.3(2)
  range-phrase=--,           % write 1--100 instead of 1 to 100
  range-units=single,        % write 1--100 GeV instead of 1 GeV -- 100 GeV
}

\DeclareSIUnit\micron{\micro\metre}
\DeclareSIUnit\rad{\radian}
\DeclareSIUnit\mrad{\milli\radian}
\DeclareSIUnit\gauss{G}
\DeclareSIUnit\eVperc{\eV\per\clight}
\DeclareSIUnit\nanobarn{\nano\barn}
\DeclareSIUnit\picobarn{\pico\barn}
\DeclareSIUnit\femtobarn{\femto\barn}
\DeclareSIUnit\attobarn{\atto\barn}
\DeclareSIUnit\zeptobarn{\zepto\barn}
\DeclareSIUnit\yoctobarn{\yocto\barn}
\DeclareSIUnit\nb{\nano\barn}
\DeclareSIUnit\pb{\pico\barn}
\DeclareSIUnit\fb{\femto\barn}
\DeclareSIUnit\ab{\atto\barn}
\DeclareSIUnit[number-unit-product = {}] \percent{\%} % remove space between number and percent sign

%%% Local Variables: 
%%% mode: latex
%%% TeX-PDF-mode: t 
%%% TeX-master: "../clicsnowmass"
%%% End: 

